The Conversation Turns First: Crowd Discussion and Price Reversals in Prediction Markets

Prediction markets combine trading with public discussion of the same events. We examine whether comment-derived signals predict subsequent activity, buying direction, and changes in the leading outcome. A correlation sweep across 79 non-political Polymarket markets guides six classification experiments comparing comment features, trading features, and their combinations. On live blocks containing comments, attention nearly matches trading history in predicting heavy trading within 18 hours (PR-AUC 0.786 versus 0.790, against prevalence 0.606), with its relative advantage concentrated in short markets. Comment content carries directional information: toxicity ranks future buying direction above chance in 43 of 53 scored markets, while adding attention, sentiment, and stance to flow history increases ROC-AUC from 0.780 to 0.788. Leadership changes are predicted primarily by market state. Stance shifts against the leader before reversals in 23 of 27 evaluable markets, but adds no clear improvement in individual-block forecasting. These results distinguish attention from directional support and price uncertainty. They establish predictive associations consistent with discussion and trading responding to shared information, without identifying a causal effect of comments on markets.

==> checklist.tex <==
\clearpage
\section*{Paper Checklist}

\subsection*{1. General research considerations}

\noindent\textbf{(a) No, not yet fully verified.} The study uses public records, but identifier handling and institutional ethics status remain unresolved.

\noindent\textbf{(b) Yes.} The abstract and introduction reflect the paper's contributions and observational scope.

\noindent\textbf{(c) Yes.} The methods support predictive comparisons, not causal claims.

\noindent\textbf{(d) Yes.} Data selection, sampling restrictions, and potential artifacts are described.

\noindent\textbf{(e) Yes.} The manuscript discusses selection bias, temporal dependence, exploratory screening, and limits to causal interpretation.

\noindent\textbf{(f) No.} Potential negative societal impacts are not explicitly discussed.

\noindent\textbf{(g) No.} Potential misuse is not explicitly discussed.

\noindent\textbf{(h) No.} Privacy safeguards, identifier handling, and a responsible data-release procedure have not been fully established.

\noindent\textbf{(i) Not yet verified.} No IRB determination was obtained; compliance with the applicable ethics guidelines has not been confirmed.

\subsection*{2. Hypotheses and theoretical considerations}

\noindent\textbf{(a) NA.} No formal theoretical results.

\noindent\textbf{(b) NA.} No formal theoretical results.

\noindent\textbf{(c) NA.} No formal theoretical results.

\noindent\textbf{(d) Yes.} The manuscript considers shared external information as an alternative explanation for observed associations.

\noindent\textbf{(e) NA.} No formal theoretical framework.

\noindent\textbf{(f) NA.} No formal theoretical results.

\noindent\textbf{(g) NA.} No formal theoretical results.

\subsection*{3. Theoretical proofs}

\noindent\textbf{(a) NA.} No theoretical proofs.

\noindent\textbf{(b) NA.} No theoretical proofs.

\subsection*{4. Machine-learning experiments}

\noindent\textbf{(a) No.} Reproduction code and data have not been released; the release decision is undecided.

\noindent\textbf{(b) No, not completely.} The main methods, splits, features, and several hyperparameters are documented, but complete reproduction details are not provided.

\noindent\textbf{(c) Yes.} Repeated-split and cross-validation results include standard deviations; a random-score control uses 200 seeds.

\noindent\textbf{(d) No.} Multiple computing environments were used, but complete hardware and compute details are not reported.

\noindent\textbf{(e) Yes.} Evaluation includes market-level holdouts, grouped cross-validation, and relevant baselines, with limitations acknowledged.

\noindent\textbf{(f) No.} Prediction metrics are reported, but practical misclassification costs are not explicitly discussed.

\subsection*{5. Existing and newly created research assets}

\noindent\textbf{(a) Yes.} Existing data, models, software, and generative-AI tools are credited.

\noindent\textbf{(b) No.} Applicable asset licenses are not comprehensively documented.

\noindent\textbf{(c) No.} The curated corpus and code are not publicly released; the release decision is undecided.

\noindent\textbf{(d) No.} Individual consent and its applicability to secondary analysis of public comments are not explicitly addressed.

\noindent\textbf{(e) No.} Identifier handling is unverified, and privacy and offensive-content considerations are not comprehensively documented.

\noindent\textbf{(f) No.} A FAIR data-release plan has not been established.

\noindent\textbf{(g) No.} No dataset datasheet is provided.

\subsection*{6. Crowdsourcing and human subjects}

\noindent\textbf{(a) NA.} No recruited participants or crowdworkers are reported.

\noindent\textbf{(b) No.} No IRB determination was obtained; the applicable review status has not been established.

\noindent\textbf{(c) NA.} No compensated participants or crowdworkers are reported.

\noindent\textbf{(d) No.} Data storage, sharing, and de-identification procedures are not fully documented; identifier handling remains unverified.

